Promoting Bright Patterns

User experience designers are facing increasing scrutiny and criticism for creating harmful technologies, leading to a pushback against unethical design practices. While clear-cut harmful practices such as dark patterns have received attention, trends towards automation, personalization, and recommendation present more ambiguous ethical challenges. To address potential harm in these "gray" instances, we propose the concept of "bright patterns" - persuasive design solutions that prioritize user goals and well-being over their desires and business objectives. The ambition of this paper is threefold: to define the term "bright patterns", to provide examples of such patterns, and to advocate for the adoption of bright patterns through policymaking.

==> archive.tex <==

% \author{Amritansh Kwatra}
% \email{ak2244@cornell.edu}
% \orcid{}
% \affiliation{%
%   \institution{Cornell Tech}
%   \streetaddress{2 West Loop Rd}
%   \city{New York}
%   \state{New York}
%   \country{USA}
%   \postcode{10044}
% }

% \author{Helen Nissenbaum}
% \orcid{}
% \email{hn288@cornell.edu}
% \affiliation{%
%   \institution{Cornell Tech}
%   \streetaddress{2 West Loop Rd}
%   \city{New York}
%   \state{New York}
%   \country{USA}
%   \postcode{10044}
% }

